An Empirical Study of Data Constraint Implementations in Java

Software systems are designed according to guidelines and constraints defined by business rules. Some of these constraints define the allowable or required values for data handled by the systems. These data constraints usually originate from the problem domain (e.g., regulations), and developers must write code that enforces them. Understanding how data constraints are implemented is essential for testing, debugging, and software change. Unfortunately, there are no widely-accepted guidelines or best practices on how to implement data constraints. This paper presents an empirical study that investigates how data constraints are implemented in Java. We study the implementation of 187 data constraints extracted from the documentation of eight real-world Java software systems. First, we perform a qualitative analysis of the textual description of data constraints and identify four data constraint types. Second, we manually identify the implementations of these data constraints and reveal that they can be grouped into 30 implementation patterns. The analysis of these implementation patterns indicates that developers prefer a handful of patterns when implementing data constraints and deviations from these patterns are associated with unusual implementation decisions or code smells. Third, we develop a tool-assisted protocol that allows us to identify 256 additional trace links for the data constraints implemented using the 13 most common patterns. We find that almost half of these data constraints have multiple enforcing statements, which are code clones of different types.

==> 000_macro.tex <==

\usepackage{amssymb}
\usepackage{ifthen}
\usepackage{comment}

\makeatletter

\newcommand{\Clarity}{{\sc Clarity}\xspace}
\newcommand{\Claritys}{{\sc Clarity's~}\xspace}


\newcommand{\tnew}[1]{{\bf { #1 }} }


\newcommand{\ndef}{\stackrel{\rm def}{=}}




\pagenumbering{arabic}




\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp \$}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }

\newcommand{\ie}{\textit{i.e.,}\xspace}
\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\etals}{\textit{et al.'s}\xspace}
\newcommand{\aka}{\textit{a.k.a.}\xspace}	
\newcommand{\secref}[1]{Section~\ref{#1}\xspace}
\newcommand{\chapref}[1]{Chapter~\ref{#1}\xspace}
\newcommand{\appref}[1]{Appendix~\ref{#1}\xspace}
\newcommand{\figref}[1]{Fig.~\ref{#1}\xspace}
\newcommand{\listref}[1]{Listing~\ref{#1}\xspace}
\newcommand{\equaref}[1]{Equation~\ref{#1}\xspace}
\newcommand{\tabref}[1]{Table~\ref{#1}\xspace}
\newcommand{\re}{\textcolor{red}{\textbf{[REF]}}\xspace}
\newcommand{\xx}{\textcolor{red}{\textbf{XX}}\xspace}

\newcommand{\stepref}[1]{Step~\ding{\number\numexpr#1+171\relax}\xspace}

\newcommand\NEW[1]{\nb{NEW}{#1}}

\definecolor{light-gray}{gray}{0.95}
\newcommand{\src}[1]{\sethlcolor{light-gray}\texttt{\small{\hl{#1}}}}
\newcommand{\srcf}[1]{\sethlcolor{light-gray}\texttt{\footnotesize{\hl{#1}}}}
\newcommand{\ttf}[1]{\texttt{\footnotesize #1}}

\newcommand{\rqa}[2]{\begin{tcolorbox}[before skip=5pt plus 2pt,boxrule=0.5pt,colframe=gray!40!white,coltitle=black,top=1pt,bottom=1pt,right=1pt,left=1pt, title=#1]{#2}\end{tcolorbox}}

\newcommand{\tcs}{187\xspace} % Total constraints
\newcommand{\tcsne}{183\xspace} % Total constraints not external
\newcommand{\cips}{30\xspace} % Total patterns
\newcommand{\freqcips}{15\xspace} % Frequent CIPs (2 or more instances)
\newcommand{\freqcipspc}{50\%\xspace} % % of cips that are frequent
\newcommand{\freqpcimp}{168\xspace} % impls that are of freq cips
\newcommand{\freqpc}{92\%\xspace} % Perc. of tcsne that are freq cips
\newcommand{\rarecips}{15\xspace} % Rare CIPs (1 instance)
\newcommand{\tdcs}{163\xspace} % Total constraints for detectors
\newcommand{\tdcscover}{87\%\xspace} % % Of const. covered by dets
\newcommand{\tps}{256\xspace} % True positives
\newcommand{\dets}{13\xspace} % Implemented detectors
\newcommand{\pcmi}{44\%\xspace} % % Of constraints with multiple implementations
\newcommand{\edscs}{159\xspace} % Constraints in expanded data set
\newcommand{\edsis}{415\xspace} % Implementations in expanded data set
\newcommand{\avgis}{2.61\xspace} % Avg impl per constraint
\newcommand{\cmi}{71\xspace} % Const with multiple impl in expanded data set
\newcommand{\tpgts}{153\xspace} % True postive ground truths
\newcommand{\arpc}{44\xspace} % Average results per constraint
\newcommand{\mrpc}{4\xspace} % Median results per constraint
\newcommand{\mars}{1,362\xspace} % Manually analyzed detector results
\newcommand{\cconsp}{93\%\xspace} % Consistent const impl (those where all instances have the same pattern)


\definecolor{typescolor}{RGB}{220,230,255}

\newcommand{\thl}[1]{\sethlcolor{typescolor}\texttt{\small\hl{#1}}\xspace}

\newcommand{\tCV}{\thl{Concrete Value}} %
\newcommand{\tVC}{\thl{Value Comparison}} % 
\newcommand{\tDVC}{\thl{Dual Value Comparison}} % 
\newcommand{\tCTV}{\thl{Categorical Value}} % 


\definecolor{patscolor}{RGB}{220,250,220}

\newcommand{\phl}[1]{\sethlcolor{patscolor}\texttt{\small\hl{#1}}\xspace}

\newcommand{\pACC}{\phl{assign class call}}
\newcommand{\pAC}{\phl{assign constant}}
\newcommand{\pBC}{\phl{binary comparison}}
\newcommand{\pBFC}{\phl{binary flag check}}
\newcommand{\pBP}{\phl{boolean property}}
\newcommand{\pCSC}{\phl{cast self-comparison}}
\newcommand{\pCA}{\phl{constant argument}}
\newcommand{\pCAs}{\phl{constructor assign}}
\newcommand{\pDC}{\phl{delta check}}
\newcommand{\pEOC}{\phl{equals or chain}}
\newcommand{\pEV}{\phl{enum valueOf}}
\newcommand{\pIC}{\phl{if chain}}
\newcommand{\pIRC}{\phl{if-return chain}}
\newcommand{\pILF}{\phl{index loop find}}
\newcommand{\pICL}{\phl{iterate-and-check literal}}
\newcommand{\pMO}{\phl{mod op}}
\newcommand{\pOVS}{\phl{override value set}}
\newcommand{\pNC}{\phl{null check}}
\newcommand{\pNBC}{\phl{null-boolean check}}
\newcommand{\pNEC}{\phl{null-empty check}}
\newcommand{\pNZC}{\phl{null-zero check}}
\newcommand{\pPM}{\phl{polymorphic method}}
\newcommand{\pPF}{\phl{properties file}}
\newcommand{\pRC}{\phl{return constant}}
\newcommand{\pSC}{\phl{self comparison}}
\newcommand{\pS}{\phl{setter}}
\newcommand{\pSE}{\phl{str ends}}
\newcommand{\pSS}{\phl{str starts}}
\newcommand{\pSwC}{\phl{switch case}}
\newcommand{\pSLC}{\phl{switch-len char}}


\usepackage{listings}
\lstset{
	frame=l,
	basicstyle=\small\ttfamily,
	numbers=left,
	language=Java
}






